COP-GEN-Beta: Unified Generative Modelling of COPernicus Imagery Thumbnails

In remote sensing, multi-modal data from various sensors capturing the same scene offers rich opportunities, but learning a unified representation across these modalities remains a significant challenge. Traditional methods have often been limited to single or dual-modality approaches. In this paper, we introduce COP-GEN-Beta, a generative diffusion model trained on optical, radar, and elevation data from the Major TOM dataset. What sets COP-GEN-Beta apart is its ability to map any subset of modalities to any other, enabling zero-shot modality translation after training. This is achieved through a sequence-based diffusion transformer, where each modality is controlled by its own timestep embedding. We extensively evaluate COP-GEN-Beta on thumbnail images from the Major TOM dataset, demonstrating its effectiveness in generating high-quality samples. Qualitative and quantitative evaluations validate the model's performance, highlighting its potential as a powerful pre-trained model for future remote sensing tasks.

==> figs/dataset-coverage.tex <==

% \begin{figure*}[tp]
    % \centering
    % \includegraphics[width=\linewidth]{images/coverage_map_train_test.png}
    % \caption{\textcolor{blue}{I think we need to improve this visualisation somehow. Blue pixels cannot be seen.} Green pixels (\textcolor{mygreen}{$\blacksquare$}) indicate the sampled locations for the training set, and blue pixels (\textcolor{myblue}{$\blacksquare$}) are locations reserved for the test set.}
    % \label{fig:dataset-coverage-train}
% \end{figure*}
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{images/coverage_map_train.png}
    \caption{Training locations are based on uniform sampling of the locations available in the union dataset of Major TOM Core for all modalities of interes.}
    \label{fig:dataset-coverage-train}
\end{figure*}

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{images/coverage_map_test.png}
    \caption{Testing locations are sparse and uniformly sampled to ensure the model has been exposed to data from all parts of the world.}
    \label{fig:dataset-coverage-test}
\end{figure*}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/discriminative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\label{tab:gen_res}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccllllllll}
\hline
Model                       & Test & \multicolumn{4}{c}{Single Modality} & \multicolumn{4}{c}{Multi-Modality}                                \\ \hline
                            &      & S1-real & S1-gen & S2-real & S2-gen & S1-real S2-real & S1-gen S2-real & S1-real S2-gen & S1-gen S2-gen \\ \hline
\multirow{2}{*}{UNet}       & real & 29.818  & 15.276 & 35.233  & 24.494 & 38.637          & 33.926         & 30.717         & 19.837        \\
                            & gen  & 13.075  & 23.556 & 16.645  & 19.496 & 16.570          & 18.172         & 15.446         & 25.526        \\ \hline
\multirow{2}{*}{RemoteCLIP} & real &         &        &         &        &                 &                &                &               \\
                            & gen  &         &        &         &        &                 &                &                &               \\ \hline
\multirow{2}{*}{DOFA}       & real &         &        &         &        &                 &                &                &               \\
                            & gen  &         &        &         &        &                 &                &                &               \\ \hline
\end{tabular}
}
\caption{mIoU}
\end{table*}

My take-aways:
 - Single modality gen experiments don't make a lot of sense
 - gen-gen experiment doesnt make a lot of sense
 - We can try: train on a mix of generated and synthetic


\begin{table*}[]
\label{tab:gen_res}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccllllllll}
\hline
Model                       & Test & \multicolumn{4}{c}{Single Modality} & \multicolumn{4}{c}{Multi-Modality}                                \\ \hline
                            &      & S1-real & S1-gen & S2-real & S2-gen & S1-real S2-real & S1-gen S2-real & S1-real S2-gen & S1-gen S2-gen \\ \hline
\multirow{2}{*}{UNet}       & real &         &        &         &        &                 &                &                &               \\
                            & gen  &         &        &         &        &                 &                &                &               \\ \hline
\multirow{2}{*}{RemoteCLIP} & real &         &        &         &        &                 &                &                &               \\
                            & gen  &         &        &         &        &                 &                &                &               \\ \hline
\multirow{2}{*}{DOFA}       & real &         &        &         &        &                 &                &                &               \\
                            & gen  &         &        &         &        &                 &                &                &               \\ \hline
\end{tabular}
}
\caption{F1 Score}
\end{table*}
